VBIT: Towards Enhancing Privacy Control Over IoT Devices

Internet-of-Things (IoT) devices are increasingly deployed at home, at work, and in other shared and public spaces. IoT devices collect and share data with service providers and third parties, which poses privacy concerns. Although privacy enhancing tools are quite advanced in other applications domains (\eg~ advertising and tracker blockers for browsers), users have currently no convenient way to know or manage what and how data is collected and shared by IoT devices. In this paper, we present VBIT, an interactive system combining Mixed Reality (MR) and web-based applications that allows users to: (1) uncover and visualize tracking services by IoT devices in an instrumented space and (2) take action to stop or limit that tracking. We design and implement VBIT to operate at the network traffic level, and we show that it has negligible performance overhead, and offers flexibility and good usability. We perform a mixed-method user study consisting of an online survey and an in-person interview study. We show that VBIT users appreciate VBIT's transparency, control, and customization features, and they become significantly more willing to install an IoT advertising and tracking blocker, after using VBIT. In the process, we obtain design insights that can be used to further iterate and improve the design of VBIT and other systems for IoT transparency and control.

==> sections/07-conclusion.tex <==
\section{Conclusion}\label{sec:conclusion}
IoT brings convenience but also introduces privacy concerns due to ubiquitous data collection. In this paper, we present \tool{}, a comprehensive and powerful approach to visualize and control, in real-time, the traffic generated by IoT devices. We provide both MR and web apps, giving users a unique perspective on their IoT device traffic and enabling greater data transparency and control. Our user study shows that \tool{} can educate users, empower them to make informed privacy decisions, and provide insights for future directions.
